Stabilized and inexact adaptive methods for capturing internal layers in quasilinear PDE

A method is developed within an adaptive framework to solve quasilinear diffusion problems with internal and possibly boundary layers starting from a coarse mesh. The solution process is assumed to start on a mesh where the problem is badly resolved, and approximation properties of the exact problem and its corresponding finite element solution do not hold. A sequence of stabilized and inexact partial solves allow the mesh to be refined to capture internal layers while an approximate solution is built eventually leading to an accurate approximation of both the problem and its solution. The innovations in the current work include a closed form definition for the numerical dissipation and inexact scaling parameters on each mesh refinement, as well as a convergence result for the residual of the discrete problem. Numerical experiments demonstrate the method on a range of problems featuring steep internal layers and high solution dependent frequencies of the diffusion coefficients.

==> ack.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Acknowledgments}
   \label{sec:ack}

MH was supported in part by NSF Awards~0715146 and 0915220,
by DOE Award DE-FG02-04ER25620,
and by DOD/DTRA Award HDTRA-09-1-0036.
JE was supported in part by XXXXXXX.



==> makefile <==
#! make
##############################################################################
# Purpose: MCP (Mathematical and Computational Physics Group) paper makefile.
#
# Notes:   This makefile is used by the MCP group (Michael Holst's Research 
#          Group in the Mathematics and Physics Departments at UC San Diego)
#          to build latex papers using the fairly simple combination of 
#          pdflatex, amstex/amslatex, and pdf/png images.
#
# Targets: The makefile will auto-generate the following based on the
#          requested make target:
#
#            Main Targets:
#
#              pdfth   --> ${TARGET}.pdf via pdflatex
#              pdf     --> ${TARGET}.pdf via pdflatex + thumbpdf
#              dvi     --> ${TARGET}.dvi via latex
#              dvip    --> ${TARGET}.dvi|ps|pdf via latex + dvips + ps2pdf
#
#            Auxilliary Targets:
#
#              arx     --> zarxiv.tar.gz (gzipped tarball for arXiv)
#              clean   --> rm -f *.aux, *.dvi, etc
#              rclean  --> clean + rm *.ps *.bbl (careful!)
#              rrclean --> rclean + rm m.pdf mm.pdf ${TARGET}.pdf (careful!)
#
# Author:  Michael Holst
# Date:    Sat Dec 19 22:23:18 PST 2009
##############################################################################

default: pdf

TARGET=dTRN15a

ARXIV_DIR=zarxiv
ARXIV_FILES=${TARGET}.tex ${TARGET}.bbl \
			environ.tex symbols.tex abs-arxiv.txt \
			abs.tex ack.tex adaptive.tex app.tex conc.tex contraction-ex.tex contraction.tex convergence.tex examples.tex intro.tex symbols.tex weak.tex

LATEX=latex
PDFLATEX=pdflatex
#PDFLATEX=pdflatex --shell-escape
BIBTEX=bibtex
#BIBTEX=./zbibtex

all : pdf arx

dvi :
	make clean
	${LATEX} ${TARGET}.tex
	-${BIBTEX} ${TARGET}
	${LATEX} ${TARGET}.tex
	${LATEX} ${TARGET}.tex
	-cp -f ${TARGET}.dvi mm.dvi

dvip : dvi
	dvips -N0 -P pdf -t letter -o ${TARGET}.ps mm.dvi
	ps2pdf ${TARGET}.ps
	-cp -f ${TARGET}.pdf mm.pdf

pdf :
	make clean
	${PDFLATEX} ${TARGET}
	-${BIBTEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	-cp -f ${TARGET}.pdf mm.pdf

pdfth : pdf
	thumbpdf ${TARGET}
	${PDFLATEX} ${TARGET}
	rm -f thumb*.png
	-cp -f ${TARGET}.pdf mm.pdf

arx : ${TARGET}.bbl
	./makex ${ARXIV_DIR} ${ARXIV_FILES}

clean :
	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt

rclean :
	make clean
	rm -f *.ps *.bbl

rrclean :
	make rclean
	rm -f m.pdf mm.pdf ${TARGET}.pdf
	rm -rf ${ARXIV_DIR}


